CF-YOLO: Context-Aware Feature Refinement for Camouflaged Industrial Micro-Defect Detection

Automated detection of surface micro-defects on industrial components, such as copper tubes, is critically important for quality assurance but remains challenging due to the minute scale of anomalies and their visual camouflage against complex backgrounds. These factors lead to weak feature representations and high rates of false positives and missed detections. To address these issues, we propose a novel real-time detection framework designed for efficient context perception and feature refinement. Our method integrates a Context-Perception Aggregation Module (CPAM), which synergises large-kernel perception for macro-texture context and small-kernel aggregation for sharp boundary delineation, effectively breaking the background camouflage. Furthermore, a Feature Additive Refinement Module (FARM) employs a linear-complexity additive token mixer to globally verify and refine the representation of fine-grained anomalies, suppressing noise-induced errors. To support research in this domain, we introduce the Copper Tube Defect Dataset (CTDD), a manually annotated benchmark containing 1,847 images and 4,898 boundingbox defect instances from copper-tube inspection scenarios. Extensive experiments demonstrate that our detector achieves strong and consistent performance on CTDD, outperforming representative baseline detectors, including YOLOv11, by 2.2% in mAP@50 and 3.9% in Precision while maintaining real-time inference speed. This work provides a robust and efficient solution for high-precision industrial inspection, bridging the gap between contextual understanding and detailed feature analysis. Our code and model are available at: https://github.com/Yu-Xinda/CFYOLO-Context-Aware-Feature-Refinement-for-Camouflaged-Industrial-Micro-Defect-Detection

==> bib.tex <==
\begin{thebibliography}{8}

\bibitem{ref_proc1}
Hwang, S., Park, J., Kim, N., Choi, Y., Kweon, I. S.: Multispectral Pedestrian Detection: Benchmark Dataset and Baseline. In: Proceedings of the IEEE conference on computer vision and pattern recognition, pp. 1037–1045 (2015)

\bibitem{ref_proc2}
Liu, J., Zhang, S., Wang, S., Metaxas, D. N.: Multispectral deep neural networks for pedestrian detection. arXiv preprint arXiv:1611.02644 (2016)

\bibitem{ref_proc3}
Konig, D., Adam, M., Jarvers, C., Layher, G., Teutsch, M.: Fully convolutional region proposal networks for multispectral person detection. In: Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition, pp.49-56 (2017)

\bibitem{ref_proc4}
Xu, D., Ouyang, W., Ricci, E., Wang, X., Sebe, N.: Learning Cross-Modal Deep Representations for Robust Pedestrian Detection. In: Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition, pp. 5363–5371 (2017)

\bibitem{ref_proc5}
Li, C., Song, D., Tong, R., Tang, M.: Multispectral pedestrian detection via simultaneous detection and segmentation. arXiv preprint arXiv:1808.04818 (2018)
\bibitem{ref_proc6}
Park, K., Kim, S.,Sohn, K.: Unified multi-spectral pedestrian detection based on probabilistic fusion networks, Pattern Recognition. 80 143–155. (2018) 
 
\bibitem{ref_proc7}
Zheng, Y., Izzat, I. H., Ziaee, S.: GFD-SSD: gated fusion double SSD for multispectral pedestrian detection. arXiv preprint arXiv:1903.06999 (2019)
\bibitem{ref_proc8}
Zhang, L.,Zhu , X., Chen, X., Yang, X., Lei, Z., Liu, Z.: Weakly Aligned Cross-Modal Learning for Multispectral Pedestrian Detection. In: Proceedings of the IEEE/CVF International Conference on Computer Vision, pp. 5127–5137 (2019)

\bibitem{ref_proc9}
Li, C., Song, D., Tong, R., Tang, M.: Illumination-aware faster R-CNN for robust multispectral pedestrian detection. Pattern Recognition. 85, 161-171 (2019)

\bibitem{ref_proc10}
Zhou, K., Chen, L., Cao, X.: Improving multispectral pedestrian detection by addressing modality imbalance problems. In: European Conference on Computer Vision, pp. 787-803 (2020)

\bibitem{ref_proc11}
Kim, J., Kim, H., Kim, T., Kim, N., Choi, Y.: MLPD: Multi-Label Pedestrian Detector in Multispectral Domain. IEEE Robotics and Automation Letters. 6(4), 7846-7853 (2021)

\bibitem{ref_proc12}
Felzenszwalb, P. F., Girshick, R. B., McAllester, D., Ramanan, D.: Object detection with discriminatively trained part-based models. IEEE transactions on pattern analysis and machine intelligence. 32(9), 1627-1645.(2010)

\bibitem{ref_proc13}
Liu, W., Anguelov, D., Erhan, D., Szegedy, C., Reed, S., Fu, C. Y., Berg, A. C.: SSD: Single Shot MultiBox Detector. In: B. Leibe, J. Matas, N. Sebe, M. Welling (Eds.), Computer Vision – ECCV 2016, Springer International Publishing, Cham, pp. 21–37 (2016)

\bibitem{ref_proc14}
Lin, T. Y., Dollár, P., Girshick, R., He, K., Hariharan, B., Belongie, S.: Feature pyramid networks for object detection. In: Proceedings of the IEEE conference on computer vision and pattern recognition, pp. 2117-2125 (2017)

\bibitem{ref_proc15}
Ronneberger, O., Fischer, P., Brox, T.: U-net: Convolutional networks for biomedical image segmentation. In: International Conference on Medical image computing and computer-assisted intervention. Springer, Cham, pp. 234-241 (2015)

\bibitem{ref_proc16}
Liu, S., Qi, L., Qin, H., Shi, J., Jia, J.: Path aggregation network for instance segmentation. In: Proceedings of the IEEE conference on computer vision and pattern recognition, pp. 8759-8768 (2018)

\bibitem{ref_proc17}
Pang, J., Chen, K., Shi, J., Feng, H., Ouyang, W., Lin, D.: Libra r-cnn: Towards balanced learning for object detection. In Proceedings of the IEEE/CVF conference on computer vision and pattern recognition, pp. 821-830 (2019)

\bibitem{ref_proc18}
Wang, X., Zhang, S., Yu, Z., Feng, L., Zhang, W.: Scale-equalizing pyramid convolution for object detection. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition, pp. 13359-13368 (2020)

\bibitem{ref_proc19}
Hu, J., Shen, L., Sun, G.: Squeeze-and-excitation networks. In: Proceedings of the IEEE conference on computer vision and pattern recognition, pp. 7132-7141 (2018)

\bibitem{ref_proc20}
Woo, S., Park, J., Lee, J. Y., Kweon, I. S.: Cbam: Convolutional block attention module. In: Proceedings of the European conference on computer vision (ECCV), pp. 3-19 (2018)

\bibitem{ref_proc21}
Dai, J., Qi, H., Xiong, Y., Li, Y., Zhang, G., Hu, H., Wei, Y.: Deformable Convolutional Networks. In: 2017 IEEE International Conference on Computer Vision (ICCV), IEEE Computer Society, pp. 764–773 (2017)

\bibitem{ref_proc22}
Carion, N., Massa, F., Synnaeve, G., Usunier, N., Kirillov, A., Zagoruyko, S.: End-to-end object detection with transformers. In: European conference on computer vision. Springer, Cham, pp. 213-229 (2020)

\bibitem{ref_proc23}
Yuan, Y., Huang, L., Guo, J., Zhang, C., Chen, X., Wang, J: Ocnet: Object context network for scene parsing. arXiv preprint arXiv:1809.00916 (2021)

\bibitem{ref_proc24}
Fu, J., Liu, J., Tian, H., Li, Y., Bao, Y., Fang, Z., Lu, H.: Dual attention network for scene segmentation. In: Proceedings of the IEEE/CVF conference on computer vision and pattern recognition, pp. 3146-3154 (2019)

\bibitem{ref_proc25}
Yang, J., Ren, P., Zhang, D., Chen, D., Wen, F., Li, H., Hua, G.: Neural aggregation network for video face recognition. In: Proceedings of the IEEE conference on computer vision and pattern recognition, pp. 4362-4371 (2017)
\bibitem{ref_proc26}
Wang, Q., Wu, T., Zheng, H., Guo, G.: Hierarchical pyramid diverse attention networks for face recognition. In: Proceedings of the IEEE/CVF conference on computer vision and pattern recognition, pp. 8326-8335 (2020)
\bibitem{ref_proc27}
Li, W., Sun, Y., Wang, J., Cao, J., Xu, H., Yang, X., Sun, G., Ma, Y., Long, Y.: Collaborative attention network for person re-identification. In: Journal of Physics: Conference Series. IOP Publishing, 1848(1), 012074 (2021)
\bibitem{ref_proc28}
Chen, B., Deng, W., Hu, J.: Mixed high-order attention network for person re-identification. In: Proceedings of the IEEE/CVF international conference on computer vision, pp. 371-381 (2019)
\bibitem{ref_proc29}
Wang, X., Girshick, R., Gupta, A., He, K.: Non-local neural networks. In: Proceedings of the IEEE conference on computer vision and pattern recognition, pp. 7794-7803 (2018)
\bibitem{ref_proc30}
Du, W., Wang, Y., Qiao, Y.: Recurrent spatial-temporal attention network for action recognition in videos. IEEE Transactions on Image Processing, 27(3), 1347-1360 (2017)
\bibitem{ref_proc31}
Su, W., Zhu, X., Cao, Y., Li, B., Lu, L., Wei, F., Dai, J.: Vl-bert: Pre-training of generic visual-linguistic representations. arXiv preprint arXiv:1908.08530 (2019)
\bibitem{ref_proc32}
Xu, T., Zhang, P., Huang, Q., Zhang, H., Gan, Z., Huang, X., He, X.: Attngan: Fine-grained text to image generation with attentional generative adversarial networks. In: Proceedings of the IEEE conference on computer vision and pattern recognition, pp. 1316-1324 (2018)
\bibitem{ref_proc33}
Mnih, V., Heess, N., Graves, A.: Recurrent models of visual attention. Advances in neural information processing systems, 27 (2014)
\bibitem{ref_proc34}
Gregor, K., Danihelka, I., Graves, A., Rezende, D., Wierstra, D.: Draw: A recurrent neural network for image generation. In: International conference on machine learning, PMLR, pp. 1462-1471 (2015) 
\bibitem{ref_proc35}

Xu, K., Ba, J., Kiros, R., Cho, K., Courville, A., Salakhudinov, R., Bengio, Y.: Show, attend and tell: Neural image caption generation with visual attention. In: International conference on machine learning,  PMLR, pp. 2048-2057 (2015)

\bibitem{ref_proc36}
Jaderberg, M., Simonyan, K., Zisserman, A.: Spatial transformer networks. Advances in neural information processing systems, 28 (2015)
\bibitem{ref_proc37}

Wang, Q., Wu, B., Zhu, P., Li, P., Hu, Q.: ECA-Net: Efficient Channel Attention for Deep Convolutional Neural Networks. 2020 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) (2020)
\bibitem{ref_proc38}
Vaswani, A., Shazeer, N., Parmar, N., Uszkoreit, J., Jones, L., Gomez, A.N., Kaiser, Ł., Polosukhin, I.: Attention is all you need. In: Advances in Neural Information Processing Systems, pp. 5998–6008 (2017)
\bibitem{ref_proc39}

González, A., Fang, Z., Socarras, Y., Serrat, J., Vázquez, D., Xu, J., López, A. M.: Pedestrian detection at day/night time with visible and FIR cameras: A comparison. Sensors, 16(6), 820 (2016)
\bibitem{ref_proc40}
Guan, D., Cao, Y., Yang, J., Cao, Y., Yang, M. Y.: Fusion of multispectral data through illumination-aware deep neural networks for pedestrian detection. Information Fusion, 50, 148-157 (2019)
\bibitem{ref_proc41}
L. Zhang, Z. Liu, S. Zhang, X. Yang, H. Qiao, K. Huang, A. Hussain, Cross-modality interactive attention network for multispectral pedestrian detection, Information Fusion. 50 (2019) 20–29.

Zhang, L., Liu, Z., Zhang, S., Yang, X., Qiao, H., Huang, K., Hussain, A.: Cross-modality interactive attention network for multispectral pedestrian detection. Information Fusion, 50, 20-29 (2019)
\bibitem{ref_proc42}
Choi, H., Kim, S., Park, K., Sohn, K.: Multi-spectral pedestrian detection based on accumulated object proposal with fully convolutional networks. In: 2016 23rd International Conference on Pattern Recognition (ICPR), pp. 621-626 (2016)
\end{thebibliography}


